Mechanistic Design and Scaling of Hybrid Architectures

The development of deep learning architectures is a resource-demanding process, due to a vast design space, long prototyping times, and high compute costs associated with at-scale model training and evaluation. We set out to simplify this process by grounding it in an end-to-end mechanistic architecture design (MAD) pipeline, encompassing small-scale capability unit tests predictive of scaling laws. Through a suite of synthetic token manipulation tasks such as compression and recall, designed to probe capabilities, we identify and test new hybrid architectures constructed from a variety of computational primitives. We experimentally validate the resulting architectures via an extensive compute-optimal and a new state-optimal scaling law analysis, training over 500 language models between 70M to 7B parameters. Surprisingly, we find MAD synthetics to correlate with compute-optimal perplexity, enabling accurate evaluation of new architectures via isolated proxy tasks. The new architectures found via MAD, based on simple ideas such as hybridization and sparsity, outperform state-of-the-art Transformer, convolutional, and recurrent architectures (Transformer++, Hyena, Mamba) in scaling, both at compute-optimal budgets and in overtrained regimes. Overall, these results provide evidence that performance on curated synthetic tasks can be predictive of scaling laws, and that an optimal architecture should leverage specialized layers via a hybrid topology.

==> _template/camera_ready_style.tex <==
\usepackage[T1]{fontenc}  
\usepackage[bookmarks=true, 
            colorlinks=true,
            linkcolor=bluegray,
            citecolor=junglegreen]{hyperref}
% \usepackage[backref=true, 
%             sorting=none]{biblatex}
%\addbibresource{./main.bib}
%\usepackage[a4paper, margin=.9in]{geometry}
\usepackage{wrapfig}
\usepackage{booktabs}  
\usepackage[bottom]{footmisc}
% \usepackage{longtable}
% \usepackage{ducksay}
% \usepackage{etaremune}
% \usepackage{afterpage}
% \usepackage{capt-of}
% \usepackage[table, x11names]{xcolor}
% \usepackage{decorule}
% \usepackage{scalerel,xparse}
\usepackage{enumitem} % customization of `list` environments
%%%% Graphics %%%%
%%%%%%%%%%%%%%%%%%

% count figures by section
\usepackage{chngcntr}
\counterwithin{figure}{section} 
\counterwithin{table}{section}

% colors and graphics
\usepackage{graphicx}
\usepackage{tikz}
\usepackage{tikz-cd}
\usepackage{hf-tikz}
\usepackage{pgfplots} 
\pgfplotsset{compat=1.17} 
\pgfplotsset{
        table/search path={figures/drawings},
    }
\usetikzlibrary{fadings}
\usetikzlibrary{shapes, arrows, fit, backgrounds, arrows.meta}

\usetikzlibrary{matrix}
\usetikzlibrary{shadows.blur}
\usetikzlibrary{patterns, tikzmark}
\usetikzlibrary{decorations.pathreplacing, calc, decorations.markings,}
\usetikzlibrary{positioning}

\usepgfplotslibrary{groupplots}
\usepgfplotslibrary{patchplots}
\definecolor{bluegray}{rgb}{0.4, 0.6, 0.8}
\definecolor{bluebell}{rgb}{0.64, 0.64, 0.82}
\definecolor{etonblue}{rgb}{0.59, 0.78, 0.64}
\definecolor{junglegreen}{rgb}{0.16, 0.67, 0.53}
\definecolor{bg}{gray}{0.97}
\definecolor{olive}{rgb}{0.6, 0.6, 0.2}
\definecolor{sand}{rgb}{0.8666666666666667, 0.8, 0.4666666666666667}
\definecolor{wine}{rgb}{0.5333333333333333, 0.13333333333333333, 0.3333333333333333}
\definecolor{deblue}{RGB}{11,132,147}
\definecolor{ocra}{RGB}{204, 119, 34}

\def\ocra{\color{ocra}}
\def\orange{\color{orange!70!white}}
\def\red{\color{red!70!white}}
\def\lblue{\color{blue!70!white}}
\def\lgreen{\color{green!70!black}}
\def\blue{\color{blue!70!white}}
\def\brown{\color{red!70!green!70!white}}

\newcommand{\fcircle}[2][red,fill=red]{\tikz[baseline=-0.5ex]\draw[#1,radius=#2] (0,0.03) circle ;}

\pgfplotsset{%
            mesh line legend/.style={legend image code/.code=\meshlinelegend#1},%
}
\makeatletter
\long\def\meshlinelegend#1{%
    \scope[%
        #1,
        /pgfplots/mesh/rows=1,
        /pgfplots/mesh/cols=4,
        /pgfplots/mesh/num points=,
        /tikz/x={(0.44237cm,0cm)}, 
        /tikz/y={(0cm,0.23932cm)},
        /tikz/z={(0.0cm,0cm)},
        scale=0.4,
    ]
    \let\pgfplots@metamax=\pgfutil@empty
    \pgfplots@curplot@threedimtrue

    \pgfplotsplothandlermesh
    \pgfplotstreamstart

    \def\simplecoordinate(##1,##2,##3){%
        \pgfmathparse{1000*(##3)}%
        \pgfmathfloatparsenumber\pgfmathresult
        \let\pgfplots@current@point@meta=\pgfmathresult
        \pgfplotstreampoint{\pgfqpointxyz@orig{##1}{##2}{##3}}%
    }%

    \pgfplotsforeachungrouped \x in {0,...,\pgfkeysvalueof{/pgfplots/samples}}{
        \pgfmathsetmacro\y{\x/\pgfkeysvalueof{/pgfplots/samples}}
        \pgfmathsetmacro\x{\x/\pgfkeysvalueof{/pgfplots/samples}*3}
        \simplecoordinate(\x,0,\y)
    }

    \pgfplotstreamend
    \pgfusepath{stroke}
    \endscope
}%
\makeatother

%%%% Fonts %%%%%%%
% Japanese Characters
% Lettrine
\usepackage{lettrine}
\usepackage{Typocaps}
\renewcommand{\LettrineFontHook}{\color{VioletRed4}\Typocapsfamily{}}
\LettrineTextFont{\itshape}
\setcounter{DefaultLines}{3}%

%%%% Theorems %%%%
%%%%%%%%%%%%%%%%%%
\usepackage{amsthm}
\newtheorem{corollary}{Corollary}[section]
\newtheorem{definition}{Definition}[section]
\newtheorem{lemma}{Lemma}[section]
\newtheorem{proposition}{Proposition}[section]
\newtheorem{remark}{Remark}[section]
\newtheorem{theorem}{Theorem}[section]
%%%% Tables %%%%
%%%%%%%%%%%%%%%%
\newcommand{\specialcell}[2][c]{%
    \begin{tabular}[#1]{@{}l@{}}#2\end{tabular}}



%%%% Table of Contents %%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage{minitoc}
\renewcommand \thepart{}
\renewcommand \partname{}

%%%% Custom cross-ref %%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\chapref}[1]{\hyperref[#1]{Chapter \ref{#1}}}
\newcommand{\secref}[1]{\hyperref[#1]{Section \ref{#1}}}


%%%% Margin notes %%%%
%%%%%%%%%%%%%%%%%%%%%
\usepackage{marginnote}
\renewcommand\raggedrightmarginnote{\sloppy}
\renewcommand\raggedleftmarginnote{\sloppy}

%%%% Boxes %%%%
%%%%%%%%%%%%%%%
\usepackage[many]{tcolorbox}
\tcbuselibrary{breakable,xparse,skins}

% add math symbols as unicode for the minted box
\usepackage{newunicodechar}
\newunicodechar{λ}{{$\mathtt\lambda$}}
\newunicodechar{μ}{{$\mathtt\mu$}}

% emphasized text
\usepackage{xparse}
\DeclareTColorBox{emphbox}{O{black}O{0cm}}{
    enhanced jigsaw,
    breakable,
    outer arc=0pt,
    arc=0pt,
    colback=white,
    rightrule=0pt,
    toprule=0pt,
    top=0pt,
    right=0pt,
    bottom=0pt,
    bottomrule=0pt,
    colframe=#1,
    enlarge left by=#2,
    width=\linewidth-#2,
}

\DeclareTColorBox{emphbox}{O{black}O{0cm}}{
    empty,
    breakable=true,
    outer arc=0pt,
    arc=0pt,
    rightrule=0pt,
    leftrule=2pt,
    borderline west={2pt}{0pt}{#1},
    toprule=0pt,
    top=0pt,
    right=-3pt,
    bottom=0pt,
    bottomrule=0pt,
    colframe=#1,
    enlarge left by=#2,
    width=\linewidth-#2,
}
\usepackage{listings}
\makeatletter
\newcommand\BeraMonottfamily{%
  \def\fvm@Scale{0.85}% scales the font down
  \fontfamily{fvm}\selectfont% selects the Bera Mono font
}
\makeatother

\lstset{
  basicstyle=\BeraMonottfamily, 
  frame=single,
}
\newenvironment{codeblock}[4][]
 {\VerbatimEnvironment
  \begin{minted}[
   mathescape,
   numbersep=5pt,
   gobble=2,
   bgcolor=gray!20,
   fontsize=\scriptsize,
   framesep=2mm,
    #1]{#2}}
 {\end{minted} 
 }

\usepackage[normalem]{ulem}

 \usepackage[draft,inline,nomargin,index]{fixme}
\fxsetup{theme=color,mode=multiuser}
\FXRegisterAuthor{sm}{asm}{\color{blue!70}SM}

==> figures/dna_loss_scaling.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{bluish}{RGB}{131,173,181}
\definecolor{greyish}{RGB}{186,60,60}

\definecolor{crimson2143940}{RGB}{214,39,40}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkorange25512714}{RGB}{255,127,14}
\definecolor{forestgreen4416044}{RGB}{44,160,44}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{mediumpurple148103189}{RGB}{148,103,189}
\definecolor{orchid227119194}{RGB}{227,119,194}
\definecolor{sienna1408675}{RGB}{140,86,75}
\definecolor{steelblue31119180}{RGB}{31,119,180}


\begin{axis}[
legend cell align={left},
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(0.03,0.03)},
  anchor=south west,
  draw=none
},
height = 4.5cm,
width = 6.5cm,
log basis x={10},
tick pos=left,
title={Compute-Optimal Scaling},
x grid style={darkgray176},
xlabel={FLOPS},
xmin=7.13000750506996e+18, xmax=8.97614763441573e+19,
xmode=log,
xtick style={color=black},
xtick={1e+17,1e+18,1e+19,1e+20,1e+21},
xticklabels={
  \(\displaystyle {10^{17}}\),
  \(\displaystyle {10^{18}}\),
  \(\displaystyle {10^{19}}\),
  \(\displaystyle {10^{20}}\),
  \(\displaystyle {10^{21}}\)
},
y grid style={darkgray176},
ylabel={PPL | Optimal Size},
ymin=3.11539126354165, ymax=3.47364139855052,
ytick style={color=black}
]
\addplot [thick, black!70, opacity=1, solid, mark=*, mark size=2, mark options={solid}]
table{%
x  y
8e+18 3.45735730150466
2e+19 3.42246683316658
4e+19 3.34413189969829
8e+19 3.30139785938991
};
\addlegendentry{Transformer++}

\addplot [thick, greyish, opacity=1, dotted, mark=x, mark size=2, mark options={solid}]
table{%
x  y
8e+18 3.40464252761469
2e+19 3.3300002756051
4e+19 3.27048409153389
8e+19 3.22813004076186
};
\addlegendentry{Mamba}

\addplot [thick, bluish, opacity=1, dotted, mark=diamond, mark size=2, mark options={solid,rotate=180}]
table{%
x  y
8e+18 3.31691082041635
2e+19 3.25485114135593
4e+19 3.20462887586443
8e+19 3.13927905156858
};
\addlegendentry{Hyena}

\addplot [thick, bluish, opacity=1, solid, mark=pentagon, mark size=2, mark options={solid}]
table{%
x  y
8e+18 3.33342986163172
2e+19 3.25162244092746
4e+19 3.20685552988592
8e+19 3.13167536058751
};
\addlegendentry{StripedHyena}

\addplot [semithick, black!70, opacity=0.75]
table {%
8e+18 3.45735730150466
2e+19 3.42246683316658
4e+19 3.34413189969829
8e+19 3.30139785938991
};

\addplot [semithick, greyish, opacity=0.75]
table {%
8e+18 3.40464252761469
2e+19 3.3300002756051
4e+19 3.27048409153389
8e+19 3.22813004076186
};

\addplot [semithick, bluish, opacity=0.75]
table {%
8e+18 3.31691082041635
2e+19 3.25485114135593
4e+19 3.20462887586443
8e+19 3.13927905156858
};

\addplot [semithick, bluish, opacity=0.75]
table {%
8e+18 3.33342986163172
2e+19 3.25162244092746
4e+19 3.20685552988592
8e+19 3.13167536058751
};

\end{axis}

\end{tikzpicture}


==> figures/loss_scaling.tex <==
% This file was created with tikzplotlib v0.10.1.

\begin{tikzpicture}[font=\small]

\definecolor{bluish}{RGB}{131,173,181}
\definecolor{greyish}{RGB}{186,60,60}

\definecolor{crimson2143940}{RGB}{214,39,40}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkorange25512714}{RGB}{255,127,14}
\definecolor{forestgreen4416044}{RGB}{44,160,44}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{mediumpurple148103189}{RGB}{148,103,189}
\definecolor{orchid227119194}{RGB}{227,119,194}
\definecolor{sienna1408675}{RGB}{140,86,75}
\definecolor{steelblue31119180}{RGB}{31,119,180}


\begin{axis}[
legend cell align={left},
legend style={fill opacity=1, font=\tiny, legend columns=1, legend image post style={scale=1}, draw opacity=1, text opacity=1, draw=lightgray204},
log basis x={10},
log basis y={10},
height = 6cm,
width = 8cm,
title style = {at={(.5, .94)}},
minor ytick={0.2,0.3,0.4,0.5,0.6,0.7,0.8,0.9,2,3,4,5,6,7,8,9,20,30,40,50,60,70,80,90,200,300,400,500,600,700,800,900,2000,3000,4000,5000,6000,7000,8000,9000},
tick pos=left,
title={Compute-Optimal~Scaling},
title style = {at={(.5, .94)}},
x grid style={darkgray176},
xlabel={\small FLOPS}, ylabel={\small PPL~$|$ ~Optimal~Size}, 
xmin=5e+18, xmax=3e+21,
xmode=log,
xtick style={color=black},
xtick={1e+17,1e+18,1e+19,1e+20,1e+21,1e+22,1e+23},
xticklabels={
  \(\displaystyle {10^{17}}\),
  \(\displaystyle {10^{18}}\),
  \(\displaystyle {10^{19}}\),
  \(\displaystyle {10^{20}}\),
  \(\displaystyle {10^{21}}\),
  \(\displaystyle {10^{22}}\),
  \(\displaystyle {10^{23}}\)
},
y grid style={darkgray176},
ymin=5.5, ymax=13.8,
ymode=log,
ytick style={color=black},
ytick={0.1,1,10,100,1000},
yticklabels={
  \(\displaystyle {10^{-1}}\),
  \(\displaystyle {10^{0}}\),
  \(\displaystyle {10^{1}}\),
  \(\displaystyle {10^{2}}\),
  \(\displaystyle {10^{3}}\)
}
]

\addplot [thick, black!70, opacity=1, solid, mark=*, mark size=1.2, mark options={solid}]
table {%
8e+18 11.269008
2e+19 9.777663	
4e+19 8.806196	
8e+19 7.855780
2e+20 6.989370
5e+20 6.310775
2e+21 5.549860
};
\addlegendentry{Transformer++}
%
\addplot [thick, greyish, opacity=1, dotted, mark=x, mark size=1.2, mark options={solid}]
table {%
8e+18 10.642644	
2e+19 9.186248	
};
\addlegendentry{Mamba}
%
\addplot [thick, greyish, opacity=1, solid, mark=triangle*, mark size=1.2, mark options={solid}]
table {%
8e+18 10.017814
2e+19 8.709058
};
\addlegendentry{+ Striping}
%
\addplot [thick, bluish, opacity=1, dotted, mark=diamond, mark size=1.2, mark options={solid,rotate=180}]
table {%
8e+18 13.66801506314
2e+19 11.0471908495558
4e+19 9.950195
8e+19 8.87140459648077
};
\addlegendentry{Hyena}
%
\addplot [thick, bluish, opacity=1, dotted, mark=diamond*, mark size=1.2, mark options={solid}]
table {%
8e+18 11.662440
2e+19 9.917158
4e+19 8.996687
8e+19 8.038690
2e+20 7.329711
5e+20 6.492402
2e+21 5.738724
};
\addlegendentry{+ Heads}
%

\addplot [thick, bluish, opacity=1, solid, mark=pentagon, mark size=1.2, mark options={solid}]
table {%
8e+18 10.025124
2e+19 8.656749		
4e+19 7.865453	
8e+19 7.190460	
};
\addlegendentry{+ Striping}
%
\addplot [thick, bluish, opacity=1, solid, mark=pentagon*, mark size=1.2, mark options={solid}]
table {%
8e+18 9.769632		
2e+19 8.414571	
4e+19 7.706391	
8e+19 7.068459		

};
\addlegendentry{++ MoE} %
%
\addplot [thick, bluish, opacity=1, dashed, mark=star, mark size=1.2, mark options={solid}]
table {%
8e+18 9.641411	
2e+19 8.239496	
};
\addlegendentry{ +++ Seq. Experts} %HyenaExperts


\end{axis}
\end{tikzpicture}

